Discrete Adjoint Momentum-Weighted Interpolation Strategies

This Technical Note outlines an adjoint complement to a critical building block of pressure-based Finite-Volume (FV) flow solvers that employ a collocated variable arrangement to simulate virtually incompressible fluids. The focal point is to strengthen the adjoint pressure-velocity coupling by using an adjoint Momentum-Weighted Interpolation (MWI) strategy. To this end, analogies of established primal MWI techniques are derived and investigated. The study reveals the merits of an adjoint MWI but also highlights the importance of its careful implementation.

==> tex/playground.tex <==
Die semi-diskrete Version von Glg. (\ref{equ:primal_momentum_balance}) basierend auf einer  state-of-the-art Finite-Volumen-Methode lautet
\begin{align}
A^P v_i^P + \sum_{NB(P)} A^{NB} v_i^{NB} = \left[ q_i - \frac{\partial p}{\partial x_i} \right]^P \Delta \Omega^P \label{equ:semi_discrete_momentum} \, ,
\end{align}
wobei $\Gamma_k^F = \Gamma^F n_k^F$ und $\Omega^P$ den Oberflächenvektor der Fläche $F$ sowie das endliche Volumen der Zelle $P$ bezeichnen. Die Einführung folgender Abkürzungen
\begin{align}
\alpha_i^P = -\frac{1}{A^P} \sum_{NB(P)} A^{NB} v_i^{NB}
\qquad \qquad \mathrm{und} \qquad \qquad
\beta^P = \frac{ \Delta \Omega^P}{ A^P} 
\end{align}
erlaubt eine kompakte semi-diskrete Bilanz ebenso für eine Nachbarzelle $B$ sowie für ein um die Fläche dazwischen (staggered) positioniertes Kontrollvolumen $F$, viz.
\begin{align}
v_i^P = \alpha_i^P + \beta^P \left[ q_i - \frac{\partial p}{\partial x_i} \right]^P \, ,
\qquad
v_i^B = \alpha_i^B + \beta^P \left[ q_i - \frac{\partial p}{\partial x_i} \right]^B  
\qquad \mathrm{und} \qquad
v_i^F = \alpha_i^F + \beta^F \left[ q_i - \frac{\partial p}{\partial x_i} \right]^F \, . \label{equ:staggered_balance}
\end{align}
Da die Zellzentren der kolokierten Kontrollvolumina mit den Flächenzentren des versetzten Gitters übereinstimmen, liefert eine lineare Interpolation einen Ausdruck für die jeweiligen Nachbarbeiträge, z.B. $\alpha_i^F = \overline{\alpha_i}^F = \lambda^F \alpha_i^P + (1-\lambda^F) \alpha_i^B$, sodass die Glgn. (\ref{equ:staggered_balance}) wie folgt zusammengefasst werden kann
\begin{align}
v_i^F = \overline{v_i^F} - \overline{\beta^F \left[ q_i  - \frac{\partial p}{\partial x_i} \right]^F} + \beta^F \left[ q_i - \frac{\partial p}{\partial x_i} \right]^F \label{equ:mwi_primal_first} \, .
\end{align}
In der Abwesenheit von Impulsquellen ($q_i \to 0$) ergibt sich das bekannte Rhie-Chow Verfahren. Weitere Vereinfachungen folgen von Realisierbarkeitsbedingungen, z.B. $\overline{\beta^F} = \beta^F$ aus \cite{bartholomew2018unified}.

Um die Interpolationsvorschrift (\ref{equ:mwi_primal_first}) auszuwerten, ist zu klären wie die jeweiligen Druck- und Volumenkraftbeiträge auf den Zellflächen bestimmt werden. Während der Druck auf der Fläche sowohl aus einem zentralen Differenzenquotienten (p, v1) als auch aus einer linearen Interpolation der anliegenden, zell-zentrierten Gradientenwerte (p, v2) folgt
\begin{align}
\frac{\partial p}{\partial x_i}\bigg|^F = \frac{p^B - p^P}{||d_k^F||} \frac{d_i^F}{||d_k^F||} 
\qquad \qquad \mathrm{und} \qquad \qquad
\frac{\partial p}{\partial x_i}\bigg|^P = \frac{1}{\Delta \Omega^P} \sum_{F(P)}  \overline{p^F} \Delta \Gamma_i^F \label{equ:discrete_grad_p_gauss} \, 
\end{align}
werden die Volumenkräfte strikt im Sinne des Gausschen-Integralsatzes Approximiert, viz.
\begin{align}
q_i^{P,v1} = \bigg[ q_i \Delta \Omega \bigg]^P
\qquad \qquad \mathrm{and} \qquad \qquad
q_i^{P,v2} = \frac{1}{\Delta \Omega^P} \sum_{F(P)} \big[ x_k^F - x_k^P \big] \overline{\overline{q_k^F}} \Delta \Gamma_i^F \label{equ:discrete_bf}, 
\end{align}
wobei ein doppelter Überstrich nun eine Distanz-gewichtete Interpolaton darstellt, z.B. $ \overline{\overline{q_i^F}} = (1-\lambda^F)q_i^P + \lambda^F q_i^B$. 
%
Drückt man Flächenzentrumskoordinaten in (\ref{equ:discrete_bf}) als eine linear interpolation der benachbarten Zellzentren ($x_k^F = \overline{x_k^F} = \lambda^F x_k^P + (1-\lambda^F)x_k^B$) aus, kann der Ausdruck weiter vereinfacht werden, cf. \cite{bartholomew2018unified}.
%
\begin{align}
v_i^F  = \overline{v_i}^F - \beta^F \left[ \left( \frac{p^B - p^P}{||d_k^F||} \frac{d_i^F}{||d_k^F||} - \overline{\overline{q_i^{v1}}}^F \right) - \left( \overline{ \frac{\partial p}{\partial x_i}}^F - \overline{q_i^{v2}}^F \right) \right] \, .
\end{align}


%\begin{align}
%\int_{\Delta \Omega (P)} \hat{q}_\mathrm{i}^\mathrm{v1} \mathrm{d} \Omega \approx \left[ \hat{q}_\mathrm{i} \Delta \Omega \right]^\mathrm{P}
%\qquad \text{und} \qquad 
%\int_{\Delta \Omega (P)} \hat{q}_\mathrm{i}^\mathrm{v2} \mathrm{d} \Omega 
%\approx 
%\sum_{F(P)} \hat{q}_\mathrm{k}^\mathrm{v2, F}\Delta \Gamma_\mathrm{i}^\mathrm{F} 
%\label{equ:discrete_bf_v1} \, .
%\end{align}

%\begin{align}
%\frac{\partial \hat{p}}{\partial x_\mathrm{i}}\bigg|^\mathrm{F,v1} = \frac{\hat{p}^B - \hat{p}^\mathrm{P}}{||d_\mathrm{k}^\mathrm{F}||} \frac{d_\mathrm{i}^\mathrm{F}}{||d_\mathrm{k}^\mathrm{F}||} 
%\qquad \qquad \text{und} \qquad \qquad
%\frac{\partial \hat{p}}{\partial x_\mathrm{i}}\bigg|^\mathrm{P,v2} = \frac{1}{\Delta \Omega^\mathrm{P}} \sum_{F(P)} \overline{\hat{p}^\mathrm{F}} \Delta \Gamma_\mathrm{i}^\mathrm{F} \label{equ:discrete_gradadp_v1_v2} \, .
%\end{align}

%\begin{align}
%\int_{\Delta \Omega (P)} \hat{q}_\mathrm{i}^\mathrm{v1} \mathrm{d} \Omega \approx \bigg[ \hat{q}_\mathrm{i} \Delta \Omega \bigg]^\mathrm{P}
%\qquad \to \qquad 
%\hat{q}_\mathrm{i}^\mathrm{v1, P} \approx \hat{q}_\mathrm{i}^\mathrm{P} 
%\qquad \text{und} \qquad 
%\hat{q}_\mathrm{i}^\mathrm{v1, F} = \overline{\overline{\hat{q}_\mathrm{i}^\mathrm{F}}} = \left( 1 - \lambda^\mathrm{F} \right) \hat{q}_\mathrm{i}^\mathrm{P} + \lambda^\mathrm{F} \hat{q}_\mathrm{i}^\mathrm{B}
%\label{equ:discrete_bf_v1} \, .
%\end{align}

%\begin{align}
%\int_{\Delta \Omega (P)} \hat{q}_\mathrm{i}^\mathrm{v2} \mathrm{d} \Omega 
%\approx 
%\int_{\Delta \Omega (P)} \frac{\partial \hat{q}_\mathrm{k} x_\mathrm{k}}{\partial x_\mathrm{i}} - \frac{\partial \hat{q}_\mathrm{k}}{\partial x_\mathrm{i}} x_\mathrm{k} \mathrm{d} \Omega 
%= 
%\sum_{F(P)} \big[ x_\mathrm{k}^\mathrm{F} - x_\mathrm{k}^\mathrm{P} \big] \overline{\overline{\hat{q}_\mathrm{k}^\mathrm{F}}} \Delta \Gamma_\mathrm{i}^\mathrm{F} 
%\qquad \to \qquad 
%\hat{q}_\mathrm{i}^\mathrm{v2, P} \approx \frac{1}{\Delta \Omega^\mathrm{P}} \sum_{F(P)} \big[ x_\mathrm{k}^\mathrm{F} - x_\mathrm{k}^\mathrm{P} \big] \overline{\overline{\hat{q}_\mathrm{k}^\mathrm{F}}} \Delta \Gamma_\mathrm{i}^\mathrm{F} 
%\label{equ:discrete_adbf_v2}
%\end{align}

%\begin{align}
    %v_\mathrm{i}^\mathrm{F} = \lambda^\mathrm{F} v_\mathrm{i}^\mathrm{NB}  + (1 - \lambda^\mathrm{F}) v_\mathrm{i}^\mathrm{P} + \overline{\frac{\partial v_\mathrm{i}}{\partial x_\mathrm{k}} \bigg|^\mathrm{F}} \left( x_\mathrm{k}^\mathrm{F} - \overline{x_\mathrm{k}^\mathrm{F}} \right)
    % o_\mathrm{k}^\mathrm{F}
    %\qquad \qquad \mathrm{with} \qquad \qquad
    %o_\mathrm{k}^\mathrm{F} = x_\mathrm{k}^\mathrm{F} - \overline{x_\mathrm{k}^\mathrm{F}}
    %- ( \lambda^\mathrm{F} x_\mathrm{k}^\mathrm{NB} + (1-\lambda^\mathrm{F} x_\mathrm{k}^\mathrm{P}) )
%\end{align}


%Comet-Like führt einen adaptiven Normalisierungswert ein, welcher nach unten hin hin hart gecoded abgeschnitten ist
%\begin{align}
%    R^\mathrm{\varphi, m} = \frac{1}{\mathrm{max}(10^\mathrm{-5},F)} \sum_\mathrm{i=1}^\mathrm{N} |r_\mathrm{i}^\mathrm{\varphi, m} |
%    \qquad \qquad \mathrm{with} \qquad \qquad 
%    F &=  \sum_\mathrm{i=1}^\mathrm{N} | r_\mathrm{i}^\mathrm{m, \varphi} \varphi_\mathrm{i}^\mathrm{m-1, \varphi}| \, .
%\end{align}
%Erfahrungen zeigen das eine derartige Normalisierung das Residuum des Druckes $R^\mathrm{p,m}$ bzw. der Druckkorrekturgleichung stark erhöht, zumindest für anfängliche Zeitschritte/Iterationen.

\section{Primal Relaxation-Free Derivation}

\begin{align}
    \left[ \frac{A}{\omega} + \frac{\rho \, \Delta \Omega}{\Delta t \, \omega} \right]^{P,t,m} v_i^{P,t,m} + \sum_{NB(P)} \left[ A \, v_i \right]^{NB,t,m} &= -\left[ \frac{\partial p}{\partial x_i} \Delta \Omega \right]^{P,t,m-1} + \left[ \frac{\rho \Delta \Omega}{\Delta t} v_i\right]^{P,t-1} \\
    &\quad + \left( 1 - \omega \right) \left[ \frac{A}{\omega} + \frac{\rho \, \Delta \Omega}{\Delta t \, \omega} \right]^{P,t,m} v_i^{P,t,m-1}
\end{align}

\begin{align}
    \left[ 1+ \frac{\rho \, \Delta \Omega}{\Delta t \, A} \right]^{P,t,m} v_i^{P,t,m} + \frac{\omega }{A}\bigg|^{P,t,m} \sum_{NB(P)} \left[ A \, v_i \right]^{NB,t,m} &= -\frac{\omega }{A}\bigg|^{P,t,m} \left[ \frac{\partial p}{\partial x_i} \Delta \Omega \right]^{P,t,m-1} \\
    &+ \frac{\omega }{A}\bigg|^{P,t,m} \left[ \frac{\rho \Delta \Omega}{\Delta t} v_i\right]^{P,t-1} + \left( 1 - \omega \right) \left[ 1+ \frac{\rho \, \Delta \Omega}{\Delta t \, A} \right]^{P,t,m} v_i^{P,t,m-1}
\end{align}

\begin{align}
    \alpha^{P,t,m} &= \frac{\omega }{A}\bigg|^{P,t,m} \sum_{NB(P)} \left[ A \, v_i \right]^{NB,t,m} \\
    \beta^{P,t,m} &= \frac{\Delta \Omega}{A}\bigg|^{P,t,m} \\
    \gamma^{P,t,m} &= \frac{\rho}{\Delta t}\bigg|^{P,t,m}
\end{align}

\begin{align}
    \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m} + \alpha^{P,t,m} &= -\omega \beta^{P,t,m} \frac{\partial p}{\partial x_i} \bigg|^{P,t,m-1} + \omega \beta^{P,t,m} \gamma^{P,t-1,m} v_i^{P,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{P,t,m}  v_i^{P,t,m-1}
\end{align}

\begin{align}
    \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m} + \alpha^{B,t,m} &= -\omega \beta^{B,t,m} \frac{\partial p}{\partial x_i} \bigg|^{B,t,m-1} + \omega \beta^{B,t,m} \gamma^{B,t-1,m} v_i^{B,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{B,t,m}  v_i^{B,t,m-1}
\end{align}

\begin{align}
    \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m} + \alpha^{F,t,m} &= -\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1}
\end{align}

\begin{align}
    \alpha^{P,t,m} &= -\omega \beta^{P,t,m} \frac{\partial p}{\partial x_i} \bigg|^{P,t,m-1} + \omega \beta^{P,t,m} \gamma^{P,t-1,m} v_i^{P,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m-1} - \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m}
\end{align}

\begin{align}
    \alpha^{B,t,m} &= -\omega \beta^{B,t,m} \frac{\partial p}{\partial x_i} \bigg|^{B,t,m-1} + \omega \beta^{B,t,m} \gamma^{B,t-1,m} v_i^{B,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m-1} - \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m}
\end{align}

\begin{align}
    \alpha^{F,t,m} &= \lambda^F \alpha^{P,t,m} + (1-\lambda^F) \alpha^{B,t,m} \\
    &= \lambda^F \left[ -\omega \beta^{P,t,m} \frac{\partial p}{\partial x_i} \bigg|^{P,t,m-1} + \omega \beta^{P,t,m} \gamma^{P,t-1,m} v_i^{P,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m-1} - \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m} \right] \\
    & \quad + (1-\lambda^F) \left[ -\omega \beta^{B,t,m} \frac{\partial p}{\partial x_i} \bigg|^{B,t,m-1} + \omega \beta^{B,t,m} \gamma^{B,t-1,m} v_i^{B,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m-1} - \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m} \right] \\
    &= -\lambda^F \omega \beta^{P,t,m} \frac{\partial p}{\partial x_i} \bigg|^{P,t,m-1} - (1-\lambda^F) \omega \beta^{B,t,m} \frac{\partial p}{\partial x_i} \bigg|^{B,t,m-1} \\
    & \quad + \lambda^F \omega \beta^{P,t,m} \gamma^{P,t-1,m} v_i^{P,t-1} + (1-\lambda^F) \omega \beta^{B,t,m} \gamma^{B,t-1,m} v_i^{B,t-1} \\
    & \quad + \lambda^F \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m-1} + (1-\lambda^F) \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m-1} \\
    & \quad - \lambda^F \left[ 1 + \beta \, \gamma \right]^{P,t,m} v_i^{P,t,m}  - (1-\lambda^F) \left[ 1 + \beta \, \gamma \right]^{B,t,m} v_i^{B,t,m} \\
    &= -\overline{\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} + \overline{\omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} + \overline{\left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1}} - \overline{\left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m} }
\end{align}

\begin{align}
    \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m} &= -\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1} \\
    &\quad + \left[ \overline{\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} + \overline{\omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} + \overline{\left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1}} - \overline{\left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m} } \right] \\
    &= -\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \overline{\omega \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \\
    &\quad + \omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} - \overline{\omega \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} \\
    &\quad + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1} - \overline{\left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m-1}} \\
    &\quad + \overline{\left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m}}
\end{align}

\begin{align}
    \left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m} &= \overline{\left[ 1 + \beta \, \gamma \right]^{F,t,m} v_i^{F,t,m}} \\
    &\quad - \omega \left[ \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \overline{\beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \right] \\
    &\quad + \omega \left[ \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} - \overline{\beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} \right] \\
    &\quad + \left( 1 - \omega \right) \left[ 1 + \beta \, \gamma \right]^{F,t,m} \left[ v_i^{F,t,m-1} - \overline{v_i^{F,t,m-1}} \right]
\end{align}

\begin{align}
    v_i^{F,t,m} = \overline{v_i^{F,t,m}} + \left( 1 - \omega \right) \left[ v_i^{F,t,m-1} - \overline{v_i^{F,t,m-1}} \right] &+ \frac{1}{\left[ 1 + \beta \, \gamma \right]^{F,t,m}} \Bigg[ -\omega \left[ \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \overline{\beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \right] \\
    & + \omega \left[ \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} - \overline{\beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} \right] \Bigg]
\end{align}

$\gamma^F \to 0$
\begin{align}
    v_i^{F,t,m} &= \overline{v_i^{F,t,m}} \\
    &\quad - \omega \left[ \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} - \overline{\beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \right] \\
    &\quad + \left( 1 - \omega \right) \left[ v_i^{F,t,m-1} - \overline{v_i^{F,t,m-1}} \right]
\end{align}

$\omega \to 1$
\begin{align}
    v_i^{F,t,m} = \overline{v_i^{F,t,m}} &+ \frac{1}{\left[ 1 + \beta \, \gamma \right]^{F,t,m}} \Bigg[ - \left[ \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} + \overline{\beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \right] \\
    & + \left[ \beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1} - \overline{\beta^{F,t,m} \gamma^{F,t-1,m} v_i^{F,t-1}} \right] \Bigg]
\end{align}

$\gamma^F \to 0$ and $\omega \to 1$
\begin{align}
    v_i^{F,t,m} &= \overline{v_i^{F,t,m}} - \left[ \beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1} - \overline{\beta^{F,t,m} \frac{\partial p}{\partial x_i} \bigg|^{F,t,m-1}} \right]
\end{align}
